Bank Density, Population Density, and Economic Deprivation Across the United States

Recent research on the geographic locations of bank branches in the United States has identified thresholds below which a given area can be considered to be a "banking desert." Thus far, most analyses of the country as a whole have tended to focus on minimum distances from geographic areas to the nearest bank, while a recent density-based analysis focused only on the city of Chicago. As such, there is not yet a nationwide study of bank densities for the entire United States. This study calculates banks per square mile for U.S. Census tracts over ten different ranges of population density. One main finding is that bank density is sensitive to the measurement radius used (for example, density in urban areas can be calculated as the number of banks within two miles, while some rural areas require a 20-mile radius). This study then compiles a set of lower 5- and 10-percent thresholds that might be used to identify "banking deserts" in various urban, suburban, and rural areas; these largely conform to the findings of previous analyses. Finally, adjusting for population density using regression residuals, this paper examines whether an index of economic deprivation is significantly higher in the five percent of "desert" tracts than in the remaining 95 percent. The differences are largest -- and highly significant -- in the densest tracts in large urban areas.

==> BDbib.tex <==
@Article{Hegerty2019a,
  author={Scott W Hegerty},
  title={{A Comparison of Tract-Level, Nationwide Indices of Economic Deprivation}},
  journal={Economics Bulletin},
  year=2019,
  volume={39},
  number={1},
  pages={256-263},
}


